Quantifying protocols for safe school activities

By the peak of COVID-19 restrictions on April 8, 2020, up to 1.5 billion students across 188 countries were by the suspension of physical attendance in schools. Schools were among the first services to reopen as vaccination campaigns advanced. With the emergence of new variants and infection waves, the question now is to find safe protocols for the continuation of school activities. We need to understand how reliable these protocols are under different levels of vaccination coverage, as many countries have a meager fraction of their population vaccinated, including Uganda where the coverage is about 8\%. We investigate the impact of face-to-face classes under different protocols and quantify the surplus number of infected individuals in a city. Using the infection transmission when schools were closed as a baseline, we assess the impact of physical school attendance in classrooms with poor air circulation. We find that (i) resuming school activities with people only wearing low-quality masks leads to a near fivefold city-wide increase in the number of cases even if all staff is vaccinated, (ii) resuming activities with students wearing good-quality masks and staff wearing N95s leads to about a threefold increase, (iii) combining high-quality masks and active monitoring, activities may be carried out safely even with low vaccination coverage. These results highlight the effectiveness of good mask-wearing. Compared to ICU costs, high-quality masks are inexpensive and can help curb the spreading. Classes can be carried out safely, provided the correct set of measures are implemented.

==> supp_materials/COMORBUSS/chapters/ch01_introduction.tex <==
% Chapter 1
\chapter{COMORBUSS} % Main chapter title
\label{Ch01} % For referencing the chapter elsewhere, use \ref{Ch00} 

COMORBUSS is a bio-social agent model for the study of disease propagation in a community and the evaluation of mitigation measures. Let us clarify each part of this statement. 

An agent model is a one where we simulate individual agents which represent persons in the modeled community. These agents interact with each other and the environment according to a set of rules, and have their own characterization. This allows for the creation of models which captures the heterogeneity of the real community we are studying. Moreover, mitigation measures can be directly modeled by modifying the behaviour of the agents (e.g. quarantines, social isolation, reduction of students in classrooms) or the transmission of the pathogen (e.g. masks and vaccination). This way, the effectiveness of these mitigation policies can be directly measured and compared, see Figure \ref{fig:effectiveness}.

By bio-social, we mean to emphasize that COMORBUSS at its core is driven by two stochastic models: one for disease progression and propagation based on the individual biology of the agents and the other for the social dynamics of the agents based on their identities and roles in the community. Connecting these two models is the core modeling assumption that disease transmission rides on social contacts produced by the community dynamics. As the social dynamics model drives the individual agents as workers or clients of the services which define the infrastructure of the community (such as hospitals, schools, markets, restaurants, stores etc.), the agents meet at these locations and possibly infect others. As transmission is contextualized by location and by the roles of the agents involved (client or worker), we can identify which are the services that contribute the most in driving the infection; see Figure \ref{fig:inf_location}.

% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Effectiveness of different mitigation policies measured by case increase relative to the scenario where the city remains in lockdown.}
%     \label{fig:effectiveness}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 0.85\textwidth]{supp_materials/COMORBUSS/figures/inf_plc.pdf}
    \caption{Percentile of infections that happen in each service category.}
    \label{fig:inf_location}
\end{figure}

COMORBUSS as an agent-based model possesses the following remarkable advantages which are derived from \textbf{our approach to directly model social dynamics} and the \textbf{omniscience the model guarantees to the analyst} :
\begin{itemize}
    \item individualized and heterogeneous description of the community;
    \item behaviour models for interventions and their quantitative assessment, even with partial compliance;
    \item realist decision making models with dynamic criteria for adoption og interventions;
    \item ability to produce counterfactual scenarios regardless of the complexity of the scenario, enabling direct comparison in experimentation;
\end{itemize}

All these advantages make COMORBUSS a valuable tool both in the evaluation of policies and in the development and testing of new ideas and methods in epidemiology.


==> supp_materials/COMORBUSS/chapters/ch02_community_model.tex <==
% Chapter 2
\chapter{Community Model} % Main chapter title
\label{Ch02} % For referencing the chapter elsewhere, use \ref{Ch00} 

\section{Creation: initializing a mimetic community model stochastically}
We seek the average epidemiological behaviour and the associate variance for a city with a given demography. This is done by simulating multiple realizations of a stochastic model for the disease propagation in this community. In order the eliminate biases introduced by a single societal network, we generate for each random seed a new community model which captures the following real demographic information of a given city:
\begin{itemize}
    \item population size;% (and density if neighbourhoods are enabled);
    \item age distribution (binned in groups of 5 years);
    \item household structure (size distribution and age distribution of members);
    \item service infrastructure;
    \item job allocation by age group.
\end{itemize}

\subsection{Creating households while preserving age distribution and average household size}

The agents are created in household groups which are defined sequentially and modified such that real age distribution and average household size are respected. In order to avoid unrealistic household structures (e.g. children living unsupervised) and to consider households with sizes far from the average, we have created and carefully curated an artificial dataset of households mimicking the households in the modelled city (see SI 3).

While the generated population is smaller than the desired population, a household is sampled from the reference population dataset. We then evaluate the average size of the households created so far: if it is smaller than the desired average household size, a new agent is added to this house; if it is  larger, an agent is randomly removed from this house. 

%While generated population is smaller than the desired population, a household is sampled from the reference population dataset. We then evaluate the average size of the households created so far, and compute the difference between the real value and the one obtained, times the number of created agents : if it is bigger than 1, a new agent is added to this house; otherwise if it is smaller than -1, an agent is randomly removed from this house. 

The probabilities used in the selection of agents to be added or removed is computed from the difference between the real age distribution and that of the current agent population. We then look at the resulting values for the age groups of the agent candidates.
\begin{itemize}
    \item If removing an agent: we consider as candidates for removal only the agents whose age groups had negative values in the difference between distributions. We then assign the absolute value of these differences to each agent and normalize them so that they sum to 1. Each value is then used as the probability of removing the corresponding agent.
    \item If adding an agent: we consider candidates for creation only agents whose age groups had positive values in the difference between distributions. We then filter these positive values and normalize them so that they sum to 1. These are used as the probabilities for selecting an agent of the corresponding age group for creation.
\end{itemize}

\begin{figure}
    \centering
    %\includegraphics{} 
    \caption{Comparison of real age distribution \textbf{according to ??} and the one obtained for a simulation according to our algorithm.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics{}
    \caption{Distribution of household size in the simulation, in agreement with the \textbf{average available in ??}.}
    \label{fig:my_label}
\end{figure}

\subsection{Household initialization of compartimental data}

In contrast to ODE simulations using compartmental data, which only require the compartment values for initialization, a bio-social agent-based simulation also requires relating compartments with social characteristics in the community. For example, in a community with $250$ individuals initialized with $5$ infectious ones, having the $5$ agents living in the same house or having them living in $5$ different houses generates very different results. In the first case, the disease cannot spread more in the same house, while in the second, it can use the time infected individuals stay at home to spread to others. While a random initialization can still be used to generate a certain tendency in simulations, the high variation in the outcomes demands several realizations in order to reduce standard deviation. Since the preferred environment for spread is always individual's homes, see {\color{red}[referencia casas]}, the average results can also be misleading. The reason is that a random initialization of few agents will most likely position only one infected agent per home. Another drawback of this approach is that it ties simulation results, and therefore calibrated parameters, to the number of agents in the community, therefore making it difficult to export results to other cities of similar but still different attributes. 

Ideally, one should be able to relate compartment data to age, social role and household distribution in a time dependent manner. This level of information would allow for a complete disassociation of the probability of infection $p$, the main parameter calibrated in this work, to the community and its individuals. Unfortunately, it is clear that such data is not available in practice, and that collecting it in a meaningful representative way would be nearly impossible. We propose a synthetic half-way solution to this problem, which consists of using data gathered from social behavior and household structure to determine the time independent probability of a given compartment structure be present at a given home. 

The technique we use to synthetically detach the calibrated infection probability $p$ from most population characteristics is to answer the following question: given a home with $n$ individuals, such that it has at least one of its members with an active compartment state, what is the chance that a given compartment configuration is present during the disease life of that home? To answer this question, let us first clear out the meaning of some of these terms:
\begin{itemize}
    \item Active compartment state: exposed or infectious states.
    \item Disease life at a home: the period of time in which at least one individual from that home is at an active compartment state. 
    \item Compartment configuration: distributing codes for each compartment, such as \verb|S|, \verb|E|, \verb|I|, \verb|R|, a configuration is any member of the combinations of $n$ codes out of the $4$ possible ones. For example, with $n=3$, the configuration \verb|SEE| tells us that the home has one susceptible person and two exposed ones. After some time, the same home can have the following configuration: \verb|SEI|, meaning that one of the exposed persons became infectious.
\end{itemize}

To determine the probability of a compartment configuration occur at a home during its disease life, we divide the time a configuration is present at that home by the total time of its disease life. We do that for as many houses as possible, averaging out the probabilities for houses with same number of people. Figure \ref{fig:exdic3ppl} shows the values we used to initialize active houses with 3 people. From the figure we deduce that, if a house with 3 people is active, and all states are possible, then the most likely configuration to occur is \verb|SSI|, with about $26.6\%$ of chance. The second most likely configuration is \verb|SSE|, with about $23\%$ of chance. The least likely configuration is the one with two exposed individuals and one susceptible one, with about $0.05\%$ of chance, and so on. Notice that a random initialization would most likely have much higher probabilities towards \verb|SSE| and \verb|SSI|, being the remaining ones not present in most realizations of the community. It is also important to mention that, when the probability of infection changes, so does the compartment configuration probabilities. In general, whenever we speak about the probability of infection in this work, we are also including inherent compartment configuration probabilities that come along with it. 

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
% Configuration & Probability \\
%  \verb|SSE| & 0.2703 \\
%  \verb|SSI| & 0.4207 \\
%  \verb|SEE| & 0.0015 \\
%  \verb|SEI| & 0.0449 \\
%  \verb|SER| & 0.0256 \\
%  \verb|SII| & 0.0369 \\
%  \verb|SIR| & 0.0828 \\
%  \verb|EEI| & 0.0035 \\
%  \verb|EER| & 0.0010 \\
%  \verb|EII| & 0.0099 \\
%  \verb|EIR| & 0.0146 \\
%  \verb|ERR| & 0.0073 \\
%  \verb|III| & 0.0075 \\
%  \verb|IIR| & 0.0241 \\
%  \verb|IRR| & 0.0494 \\
%     \end{tabular}
%     \caption{Compartment configuration probabilities used for active homes occupied by tree people}
%     \label{tab:exdic3ppl}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{supp_materials/COMORBUSS/figures/ch02/3pplHouseConfProb.pdf}
    \caption{Compartment configuration probabilities used for active homes occupied by tree people}
    \label{fig:exdic3ppl}
\end{figure}

The compartment configuration probabilities should be approximately the same for any point in time, and they also should not depend on the population number, only its household structure and overall social behaviour. As a result, we can safely use these probabilities to distribute compartment labels to individuals of a randomly selected active home, for as long as there are active compartment labels to distribute. After all active compartment labels are distributed, we randomly select houses to contain a given proportion of susceptible and recovered individuals. This proportion is also estimated from homes which have ended its disease life, therefore not containing active compartment individuals. 

Although the procedure just described allows for a consistent initialization of compartment states along homes in a community, collecting the data necessary to do so is still a hard task. However, if we suppose that the overall social behavior of the community is well captured, and also that the disease modelling inside homes is realistic, then we can conclude that the probability of infection itself determines the probability of each compartment configuration occur at an active home. This is the argument that allows us to use COMORBUSS to determine the compartment configuration probabilities. The idea is that, in order to simulate a community for a given probability of infection $p$, we first use another simulation to determine the compartment configurations for each possible size of a home. That is, we perform many realizations of a community disease spread using random initialization of states first. Next, we use houses whose disease life is fully captured by the simulations to determine the probabilities for each compartment configuration. Once these probabilities are derived, they are used to initialize compartment states of a second simulation, being that the one that approaches the real life's initial spread the most.


\subsection{Service infrastructure and job allocation}
Each service category (e.g. hospitals, supermarket, schools etc.) is created as a computer object sharing common defining and operating parameters. Inside each of these objects, we instantiate the same number of these service locations as are known to be had by the modelled city. One of the defining parameters is the average number of workers in the service category and the age groups that are known to function as workers. From this, when the service is created, we randomly select agents in the population of the appropriate age group and assign them as workers for that service. More detailed assignment procedures are in principle possible but are unavailable due to lack of required data. 

\section{Dynamics: stochastic model for community behaviour}
\subsection{Services as community drivers}
The core concept of COMORBUSS is the utilization of services to dynamically generate contacts in our model community. As such, each relevant social context is modelled as a service, even "the environment" as is dubbed random meetings on the streets and parks. The services which have been modelled in this work are
\begin{itemize}
    \item health facilities: hospitals, USFs (public health clinics);
    \item educational facilities: schools and day-cares;
    \item essential stores: street fairs, markets, supermarkets, food stores, construction stores;
    \item city hall and environment.
\end{itemize}
\noindent The full list of the parameters which define a service is given and explained in the next section. 

An agent can have one of three roles when inside a service: it can be a worker, a visitor or a guest (someone whose standard address has been temporarily set to the service, due to hospitalization or quarantine). Every agent is assigned as a visitor to an instance of the service categories that it can visit. This agent will always visit the same instance, unless it is temporarily reassigned to a new instance. This can happen when a service is closed due to lack of workers (all workers being in quarantine or hospitalized). Visitors can in principle be assigned to multiple instances of that service class (e.g. visit more than one supermarket), but there was no reliable data sources upon which we could model more complex behaviour.

Each service has two defining restrictions: its working days and hours, as well as the age groups allowed to use it. Another key parameter is the average period of visitation for that service (e.g. one can say that any person visits the supermarket every week). From this we have the average frequency in days that the service is visited and, using the number of working hours of that service, we compute the hourly probability that an agent will visit that service.

During every hour a service is open, free visitors are randomly selected and sent to the instance of that service they are assigned to. If the agent is unable to make a visit (e.g. agent is working or visiting another service), the probability is accumulated to a later hour that the service is open and the agent is available to visit. In this way we organically produce "rush hours", such as when many workers visit the supermarket after their working hours. After concluding its visits, the agent is then returned to its address until it is selected again for some other activity.

Similarly, workers are sent to the instance of the service where they work during their working hours. One can also allocate the agents uniformly on different shifts. Guests are so far defined only via hospitalization or quarantines, so their mobility is restricted until the associated measure is completed. They are then returned to their household address, where normal social activities are resumed.

In this way, agents are driven between different locations and contexts according to their individual needs. At the same time, the collective behavior of the agents produces a complex and realistic model for the community dynamics. Any non pharmaceutical intervention can be modelled as temporary changes in the individual or collective behavior of the agents and its consequences can be measured directly.

\subsection{Estimating visitation periods}

Letting aside the interaction of agents inside the service for a moment, the visitation of agents is what contributes the most for the relevance of services in the disease spreading at the community. COMORBUSS models the visitation of agents to a service by randomly picking them according to a probability $p_{v}$. This happens at every time step that the service is opened and that agents are free for visitation, meaning that they are not resting at home nor visiting any other service. The probability $p_{v}$ is then given by the inverse of the visitation period $v_p$: $p_{v}=1/v_p$, where $v_p$ is a measure of how many time steps an agent takes to return to a service, given that it is opened\footnote{A direct implication of this definition is that the visitation period cannot have time length lesser than that of a time step}. To make the visitation period independent on the opening of the service and also on the magnitude of time steps, we assume that it is provided in consecutive days, and then we convert it to time steps. The conversion formula is given by 
\begin{equation}
    v_p = \frac{d_o}{7}\frac{h_o}{\Delta t}v_{pc},
\end{equation}
where $d_o$ is the total number of days a service is opened on a week, $h_o$ is the total number of hours a service opens for a day, $\Delta t$ is the time step in hours, and $v_{pc}$ is the visitation period in consecutive days. To calculate $v_{pc}$, it suffices to know the total number of visitors $v_w$ a service receives during a week, and the total number of agents $v_t$ that can in fact visit the service. With these two values the visitation period in consecutive days is given by 
\begin{equation}
    v_{pc} = 7\frac{v_t}{v_w}. 
\end{equation}

We now show the how visitation periods have been estimated for different services.

%\subsection{Estimation of visitation periods}

\subsubsection{Street market}

Street market opens at Saturdays, from 6:00 to 12:00. During the pandemics, an average of $3000$ people visited the street fair every day it opens, {\color{red}see Section~\ref{sec:maragogi_is_typical}}. Assuming that all people from age groups 5 and above can visit the fair, the calculation for $v_{pc}$ is 
$$
v_{pc} = 7\frac{v_t}{v_w} = 7\frac{20884}{3000} \approx 48.73 ~\mathrm{days}. 
$$

\subsubsection{Hospitals}

% The campaign hospitals that mainly received people with COVID-19 symptoms are UPA and SAMU. 
The total number of hospital attendances in each unit of hospital (UPA and SAMU) from April, 29th to June, 28th 2020 was $3579$ and $304$, respectively. To estimate the actual number of people who visited the hospitals during this period of time, we must take into account other people accompanying these attendees. In order to do that, let us suppose that at least children from the first 3 age groups are accompanied by an adult, and that the same happens to elderly from the 13th age group and above. 

Assuming that everyone in Maragogi had the same number of contacts with the disease, we estimate from the susceptibility $p_{sus}$ and the probability of developing severe symptoms $p_{sev}$, what is the portion $po$ of attendees that brought another person with them to the hospital:
$$
po = \frac{\langle p_{sus} * p_{sev} ,pop_{ce}\rangle }{\langle p_{sus}*p_{sev},pop_{t}\rangle } \approx 0.2496,
$$
where $*$ is the point-wise multiplication of vectors, $\langle \cdot , \cdot \rangle$ is the inner product, $pop_{t}$ is the vector of all people from all age groups, and $pop_{ce}$ agrees with $pop_t$ for children or elderly, but has null entries otherwise. 

The attendees of UPA do not all come from Maragogi, but the hospital estimates that at least half of them do. Taking all this information into account, we estimate the visitation to the hospitals to be
$$
v_{pc} = (180-120)\frac{32702}{(0.5*3579+304)*1.2496} \approx 750 ~\mathrm{days}.
$$

\subsubsection{USFs}

The USFs opened during the week only, but they receive much more people. From the day 130 to 210 of 2020, they have attended a total of $7334$ people. Taking into account people that come accompainged, the visitation period for the USFs is
$$
v_{pc} = (210-130)\frac{32702}{7334*1.2496}\approx 285.5
$$

\subsubsection{Supermarkets}

To account for visitation routines in supermarkets, $5$ of the largest of its kind have been interviewed. The supermarkets ``Preço bom'' have reported $3000$ attendances every week, while supermarkets ``Supermar'', ``Mercado Nacional'' and ``Mercadinho Durare'' have reported an average of $550$ attendances weekly. As a result, the visitation period for this category of services in days is
$$
v_{pc} = 7\frac{20884}{3550} \approx 41.18,
$$
as long as all age groups from the fifth and above are considered consumers. 

\subsubsection{Markets}

Given the big difference in the contact network for supermarkets and other kind of markets, we decided to separate them into two distinct types of service. For markets, which are more local and smaller in size, we gathered information from two representatives, namely markets ``Mini Carrefour'' and ``Mercadinho do Beto''. These two markets reported an average of $50$ visitors per week. We then assumed similar visitation for all other $37$ instances, which then allowed us to estimate the following visitation period, in days:
$$
v_{pc} = 7\frac{20884}{50*39} \approx 74.97.
$$

\subsubsection{Food Stores and Construction stores}

The other types of services that received people and that remained opened during the period considered were grouped into two categories: 
\begin{itemize}
    \item Food stores: all other types of services that sell specialized food, such as fruits and vegetables and beverages. This category also includes pharmacies. 
    \item Construction stores: all types of stores sells maintenance equipment, such as those for civil engineering, household equipment, vehicle parts, etc.
\end{itemize}
These two types of stores are small and we assumed their visitation periods were twice and four times longer than the visitation period of markets, respectively. 


\section{Location contextualized contact networks}
By collecting the list of visitors, workers and guests at an instance of a service at any given time, we naturally know the collective history of the community and the sets of agents that can interact. However, how these agents interact is closely associated with the social context at that time. As examples: one does not interact closely between tables in a restaurant while the waiter interact with the set of tables it is responsible for as well as coworkers; in a classroom or factory, people are rigidly placed in space for most of the time. 

We therefore need to consider the social context of the agents in the process of taking the list of agents in a location and producing a contact network. COMORBUSS identifies each particular service having its own network structure, so distinct network models are built when representing restaurants, markets, hospitals or schools.

All network models share as a common feature to contain in each service two types of individuals: \emph{workers} and \emph{guests}. \emph{Workers} of a particular service are individuals which stay in this service over a daily time period during a realization of the stochastic community. On the opposite, \emph{guests} are individuals which visit a single time step that service respecting a frequency of visitation over the simulation. 

Both types of individuals are specialized for each service to mimic realistic features one may find in real-world services. For instance, waiters in restaurants are modelled as workers having contacts with visitors. The same idea is applicable to cashiers in markets. Hence, these observations also must be taken into account in the modelling of contact networks. Below we detail the network model for each service.

\subsection{Standard networks: houses and generic services}

In houses or generic services, no network configuration can be assumed. As a result, we utilize a standard network model in order to generate contacts. The contacts in this model are randomly distributed for each agent according to a given average number. This average value may change as the number of agents increase or decrease inside services, as discussed in Section \ref{sec:aggl}. Nevertheless, the contact networks generated are still dynamic, varying as agents are added or removed.

The contact networks are, with few exceptions, generated using Erdos-Renyi model, where the probability
$p_{ER}$ of an edge being added is given by $p_{ER} = c_{avrg} /(N − 1)$. Here $c_{avrg}$ is the average number of contacts and $N$ is the total number of nodes in the graph. The parameter $c_{avrg}$ depends on the definition of contacts, and in this work we assume it to be the following: “two people at two meters or less away from each other for the duration of one hour”. 

\subsection{Contact varying with agglomeration}\label{sec:aggl}

Each of the contact networks exposed in the sections below assume a fixed number of agents in order to distribute contacts at a given time step. However, this number may vary along time steps for several reasons. For example, in the case of markets, there are rush hours in which agglomeration is higher. It is also common in this type of service that visitors visit less in the first hours of the day, as well as in the last ones. To deal with the non-uniformity of the number of agents inside each service, we propose a formula to adjust the average number of contacts. The idea comes from supposing that the opportunity for a contact is directly linked to the available space to the agents.

Suppose that two of $N$ agents get in contact with each other whenever they share some specified area $A$ around their position in space. The expression relating $c_{avrg}(N)$, $A$ and $N$ is given by
\begin{equation}\label{eq:rand_walk_avrg_cont}
    E(c_{avrg}(N)) = \frac{\frac{N(N-1)}{2}A}{N} = \frac{N-1}{2}A,
\end{equation}
where $E$ is the expectation operator. This formula comes from assuming random walking of $N$ agents inside a given service with transit area $A$. To avoid knowing the transit area, we suppose that a sample $N_0$, $c_{avrg,0}:=c_{avrg}(N_0)$ is collectable, and then we approximate $A$ through the formula
\begin{equation}
    A\approx \frac{2c_{avrg,0}}{N_0-1}.
\end{equation}
As a result, the expression for the mean number of contacts $c_{avrg}(N)$ varying with the number of agents $N$ is  
\begin{equation}\label{eq:aggl_cont}
    c_{avrg}(N) \approx c_{avrg,0}\frac{N-1}{N_0-1}.
\end{equation}

Equation \eqref{eq:aggl_cont} is used in some of the contact networks introduced below. For example, in the case of markets, supermarkets or street markets, the formula can be used to adjust the average number of contacts among visitors shopping in the services. In the case of hospitals, the formula can be used in the average number of contacts among visitors. Another place where such expression is useful is in the contact network for homes. Assuming equally sized homes, one can infer that the more people at home, the more contacts. Since the number of people at home varies along the day, such formula is well fitted to capture the dynamics of movement inside a home. 


\subsection{Networks for environment layer}

The dynamic of contacts in environment layers is very individual-specific, and therefore we approximate it by random walking. The formula for the average number $c_{avrg}$ of contacts among $N$ agents in the environmental layer with transit area $A$ is given by equation \eqref{eq:rand_walk_avrg_cont}. The transit area $A$ is in this case given by:
\begin{equation}
    A = \frac{\pi r^2}{A_u},
\end{equation}
where $r$ is an \textit{infection radius}, and $A_u$ is the urban area available in the environment layer. The infection radius is given by half of the largest distance between two agents such that they can be considered to be in contact. We assume $2$ meters as a default value.

Although at random, contacts may follow some tendency according to the age of agents. We have used the probabilities exposed in Figure \ref{fig:waifw}, which have been derived from Table 2 of \cite{DelValle2007}.


\begin{figure}
    \centering
    \includegraphics[scale=0.8]{supp_materials/COMORBUSS/figures/ch02/waifw.pdf}
    \caption{Color map representing probabilities that if a person from an age group in the y-axis met someone, that person belongs to the age groups in the x-axis.}
    \label{fig:waifw}
\end{figure}

\subsection{Network for restaurants}

Waiters are restaurant workers who have the greatest potential of becoming disease super spreaders inside their work place. This happens because they get in contact, as a group, with every visitor who enters the restaurant. As a result, waiters define a special group of workers which must have special treatment regarding their contact network.

Taking into account the social roles of waiters in restaurants, we model contacts in three categories:
\begin{itemize}
    \item \emph{visitor-visitor} contacts. 
    \item \emph{waiter-visitor} contacts. 
    \item \emph{worker-worker} contacts.  
\end{itemize}

Having these categories in mind, the contact networks for restaurants are configured by setting the following parameters: the portion of workers who are waiters, the average number of contacts among workers, and the mean number of persons seating around the same table. Because this last parameter is usually difficult to estimate, it can be discarded, in which case tables are evenly distributed among waiters in the restaurant. 

The contact network for workers is randomly created, always respecting the mean number of contacts provided as input. Among these workers are those composed of waiters, who get in contact with every visitor on the tables they serve. These visitors in turn get in contact with everyone else in the same table. 

Figure \ref{fig:rest_net} shows an example of a network for a given restaurant with $5$ visitors, $2$ waiters and $3$ other workers. Notice that only the waiters, identified by ids $1878$ and $867$, are those who get in contact with the visitors. It is clear, however, that other workers get in contact among themselves. The same thing happens to visitors in the same table.

\begin{figure}
    \centering
    \includegraphics{supp_materials/COMORBUSS/figures/ch02/rest_net.pdf}
    \caption{Example of a dynamic network for restaurants. Agents (with their ids in circles) in red are workers, agents in blue are visitors. Numbers inside each circle represent the identification number of that agent.}
    \label{fig:rest_net}
\end{figure}

\subsection{Network for markets}

The contact network for markets is similar to that of restaurants in the sense that there exists a class of workers which needs different treatment: the cashiers. While other workers usually do not get in contact very frequently with visitors, every visitor mandatorily gets in contact with a cashier, either directly or indirectly through shared surfaces, such as shopping belts or credit card machines. Second order contacts include those among visitors and among workers. 

The contacts between workers and visitors is randomly created, respecting a given average of contacts provided as input. The contacts between visitors and cashiers is also random, but in this case each visitor is assigned to a cashier. Cashiers are fixed agents, which comprise a fixed proportion of all workers in markets. 

Figure \ref{fig:market_net} shows an example of a network for a market. Notice that every visitor (blue agent) gets in contact with at least one worker. Cashiers are workers (red agents) who get in contact with many visitors. Example of cashiers in the figure are those with ids $1479$ and $9059$. Example of non-cashiers are those with ids $1922$ and $2059$

\begin{figure}
    \centering
    \includegraphics{supp_materials/COMORBUSS/figures/ch02/market_net.pdf}
    \caption{Example of a dynamic network for markets. Agents (circles) in red are workers, agents in blue are visitors. Numbers inside each circle represent the identification number of that agent.}
    \label{fig:market_net}
\end{figure}

\subsection{Network for schools}

Schools have two different network models: one for class time, and one for break time. During classes, the nature of contacts among students can be very geographic, since students tend to stay seated during long periods of time. During breaks, students are free to walk around public spaces inside the schools. As a result, the distinction between two types of networks is needed. 

During class time, we propose a network that connects agents according to the neighbors nearby, where students are assumed to follow a geographical disposition of a rectangle. Teacher are treated separately, since they usually move more frequently. The contact frequency between a student and a teacher may vary according to the age of the student. For example, for students who are toddlers, the contact is frequent, but for university students, direct contacts are unusual. The parameters for this type of network are the number of students in a class, and the average number of contacts between teachers and students.

During break time, we propose a simple network in which students get in contact at random. The factor that influences the most this type of network is the number of classes allowed to have a break together, as well as the different ages of the students. The parameters for this network are the number of classes to have break together and the average number of contacts among students. 

Figure \ref{fig:schools_net} shows a network for classes inside a school. The teacher is identified by the id $1772$.

\begin{figure}
    \centering
    \includegraphics{supp_materials/COMORBUSS/figures/ch02/schools_net.pdf}
    \caption{Example of a dynamic network for classes in schools. Students are geographically positioned in lines, with one teacher in charge.}
    \label{fig:schools_net}
\end{figure}

\subsection{Network for hospitals}

Networks for hospitals have, in addition to workers and visitors, admitted persons (hereby labelled guests), which stay in the facility for long periods of time. While these people are admitted, they get in contact with only a few hospital workers. The workers, on the other hand, get in contact with other workers, with some getting in contact with visitors as well. Visitors are yet another type of individuals which comprise those who seek help in the occasional sickness, as well as those only visiting admitted persons. The need to distinguish between three types of agent makes this type of network more complex than those introduced before. Another source of complexity is the fact that some workers are assigned to deal with a specific disease in a pandemic scenario, an attempt to contain the spread of the disease among workers. 

Contacts for visitors are adjusted by providing the average number of contacts among themselves, to the workers of the hospital, and to the admitted persons. Contacts among workers take into account the two classes of workers: typical workers and disease workers. The average number of contacts among typical workers, among disease workers, and between typical workers and disease workers must be provided. This last number is typically very small. Finally, the average number of contacts between admitted persons and disease workers is a key parameter, which can determine the spread of the disease in the hospital. 

Figure \ref{fig:hosp_net} exemplifies the network for hospitals. Agents with ids $567$, $7372$, and $4955$, in purple, have been admitted to the hospital. Agents $9943$, $7828$ $9345$ are disease workers, the only workers to get in contact to the admitted people. However, they may as well get in contact with other workers, in the figure, exemplified by the contact between agent $9345$ and agent $435$. This last worker may get in contact with another worker, exemplified by its connection to agent $1132$. Workers also get in contact with visitors, which can be seen by the connection between agent $435$ and agent $8391$. Finally, several visitors (in blue), also get in contact among themselves, as exemplified by the connection between agent $517$ and agent $9300$.

\begin{figure}
    \centering
    \includegraphics{supp_materials/COMORBUSS/figures/ch02/hosp_net.pdf}
    \caption{Example of a dynamic network for hospitals. Agents (circles) in red are workers, agents in blue are visitors, and agents in purple have been admitted to the hospital. Numbers inside each circle represent the id of that agent.}
    \label{fig:hosp_net}
\end{figure}

\section{Service parameters}
Every service is defined by the following parameters:
\begin{itemize}
    \item \verb|name|: Name of the service;
    \item \verb|number|: Number of instances of this service;
    \item \verb|days|: Days of the week the service is open to visitation;
    \item \verb|hours|: Hours of the day the service is open to visitation;
    \item \verb|visitation_period|: Mean period in days each agent visits this service;
    \item \verb|age_groups|: List of age groups that visits this service;
    \item \verb|workers|: Parameters to select workers of different types in this service. Each type can be configured with:
    \begin{itemize}
        \item \verb|name|: Name of the worker type;
        \item \verb|number|: Number of this worker type by instance;
        \item \verb|shifts|: Shifts available for this type of worker, workers are uniformly distributed between shifts;
        \item \verb|age_goups|: List of age groups that can be this worker type.
    \end{itemize}
    \item \verb|rooms|: Rooms to distribute workers, each room type is defined with a fixed number for each worker type, rooms of each type are created until there is no more workers of the required type available. At the end all remaining workers are placed in the "public" room that is the same room used by visitors;
    \item \verb|net_type| and \verb|net_par|: Type of network and it's parameters to be used to generate contacts in this service;
    \item \verb|inf_prob_weight|: Weight applied to the infection probability in this service (used to reduce the infection probability in outdoor services);
\end{itemize}

==> supp_materials/COMORBUSS/chapters/ch03_epidemiologic_model.tex <==
% Chapter 3
\chapter{Epidemiological Model} % Main chapter title
\label{Ch03} % For referencing the chapter elsewhere, use \ref{Ch00} 

\section{Progression: stochastic compartmental model for the disease}
At any time, the state of an agent with respect to the modeled disease falls into one of the following compartments:
\begin{itemize}
    \item ($S$) Susceptible: the susceptible portion of individuals in the population. This portion of the population comprehends persons that had never had contact with the disease, and therefore they are susceptible to an infection.
    \item ($E$) Exposed: the exposed (or incubating) portion of individuals in the population. Individuals in this scenario have already had contact with the disease, but are still in the incubation stage of the disease. This means that they had been infected but are not infectious.
    \item ($I$) Infectious: the agent carries the virus and is infectious. The disease itself can manifest in different ways, which are sub-categorized as: 
    \begin{itemize}
        \item ($P_s$) Pre-symptomatic: particles have already become infectious, but they have not yet developed a viral load large enough to show symptoms.
        \item ($A_s$) Asymptomatic: this type of particle has passed activation of the disease, but will never show symptoms. However, they are still infectious.
        \item ($S_y$) Symptomatic with mild symptoms: the population in this portion are those infectious that show mild symptoms.
        \item ($S_s$) Symptomatic with severe symptoms: the population in this portion are those infectious that show severe symptoms.
    \end{itemize}
    \item ($R$) Recovered: the recovered particles have gone through all the stages of the disease, and that had overcome the disease.
    \item ($D$) Deceased: the deceased particles have gone through all the stages of the disease, developed severe symptoms and that have died due to it.
\end{itemize}

Upon contracting the virus (becoming exposed), agents follow the transitions diagram depicted in Figure \ref{fig:state_transition}. The transition between states is stochastic, with transition probabilities as the inverse of the average period on which people remain in that compartment, according to the literature. {\color{red}The values and references for these periods are organized in Table}. After becoming infectious, an agent remains pre-symptomatic for two days, after which there is the activation event when it is decided if the disease will manifest as asymptomatic or symptomatic with mild or severe symptoms. {\color{red} The choice during activation is random and respects the distribution of cases according to . Infectious agents recover with a probability estimated from the average duration of the infection; note that the duration of the disease in the case of severe symptoms is longer and such agents can instead convert to the Deceased compartment with a probability dependent of the age group of the agent according to }.

\begin{figure}[]
    \centering
    \includegraphics[width=0.7\textwidth]{supp_materials/COMORBUSS/figures/ch03/inf_chain.pdf}
    \caption{Caption}
    \label{fig:state_transition}
\end{figure}

\section{Transmission}
\subsection{Standard: contact through location-contextualized network}
The standard transmission model for COMORBUSS is based on the contact networks in a location. The first condition for transmission is that a susceptible agent be in contact with an infectious one. Provided such a meeting happens, the susceptible agent converts to the exposed compartment if a random number drawn from a uniform distribution (in unit interval) is less of equal than then probability of an infection occurring. This probability is the product between the infection probability which is produced by the calibration of the model, the susceptibility of the susceptible agent (which depends on its age group and vaccination status) and a correction parameter which accounts for contacts that do not last the entire time step of an hour.

If this random decision process results in a new infection, the compartment of the previously susceptible agent is rewritten to exposed, and the location, time and source of the infection are recorded in an infection tree.

\subsection{Specialized: aerosol transmission model in indoor locations}
In many closed locations where people are present for long periods of time, the main form of infection is not via direct contact with an infections person, but by inhaling infectious particles which are suspended in the air and accumulate over time. Naturally, the modeling of this process requires more detailed information on that location, as it depends on its volume and its rate of air exchange with the outside. These details are not readily available for most services, but for the purposes of this study we acquired the data of the two major schools in the modeled city. 

We developed a modified Wells-Riley model which takes into account different parameters for teachers and students. Not only do we consider that these two groups may have different masks, but teachers also release more infectious particles since they speak loudly and continuously. {\color{red}The modeling details are provided in }.

COMORBUSS naturally tracks all the agents in each classroom and identifies which are infectious. By solving a differential equation for the concentration of infectious particles over time, we compute the balance of absorbed and released particles by students and teachers. We then compute the dose absorbed by each agent in the last time step, and from this dose we evaluate the probability of that agent being infected. {\color{red} Please check SI QQQ for the formulas involved in this procedure}. Once an infection is produced, we randomly select a source among the infectious individuals in that room and store all the details of this new infection and the usual infection tree.


\section{Disease-defining Parameters}

\begin{itemize}
    \item \verb|inf_probability|: Probability of an infectious particle to pass the infection in an encounter.
    \item \verb|susceptibility|: Susceptibility of an particle (defined by age group), the final probability of an infection to occur in an encounter will be given by the \verb|inf_probability| of the source particle multiplied by the \verb|susceptibility| of the susceptible particle.
    \item \verb|inf_duration|: Mean duration of a asymptomatic or mild symptomatic infection (infectious state).
    \item \verb|inf_severe_duration|: Mean duration of a severe symptomatic infection (infected state).
    \item \verb|inf_incubation|: Mean duration of the incubation period (exposed state).
    \item \verb|inf_sympt_timeto|: Time between the the transition to the infectious state and the activation of symptoms.
    \item \verb|inf_prob_sympt|: Probability of a infected particles to develop symptoms (defined by age group).
    \item \verb|inf_severe_sympt_prob|: Probability of a infected particles to develop severe symptoms (defined by age group).
    \item \verb|inf_severe_death_prob|: Probability of a infected particles to die (defined by age group).
    \item \verb|inf0_perc| ??? : Percentage of particles in each infection compartment at the start of the simulation. This is obtained from sampling of the distribution of cases in the initial step inferred in the calibration process.
    \item \verb|inf0_perc_symp| ??? : Percentage of infected particles in each symptoms compartment at the start of the simulation.
\end{itemize}

\begin{table}[]
\begin{tabular}{lll}
\textbf{Parameter}                             & \textbf{Used value}                                                                                                                                                    & \textbf{Source}                               \\
\verb|inf_probability|         & 0.1105                                                                                                                                                                 & Calibration                                   \\
\verb|susceptibility|           & {[}0.34, 0.34, 0.34, 1., 1., 1., 1., 1., 1., 1., 1., 1., 1., 1.47, 1.47, 1.47, 1.47, 1.47, 1.47, 1.47, 1.47{]}                                                         &                                               \\
\verb|inf_duration|            & 8.0                                                                                                                                                                    &                                               \\
\verb|inf_severe_duration|    & 14.0                                                                                                                                                                   &                                               \\
\verb|inf_incubation|          & 4.6                                                                                                                                                                    &                                               \\
\verb|inf_sympt_timeto|       & 1.8                                                                                                                                                                    &                                               \\
\verb|inf_prob_sympt|         & {[}0.5, 0.5, 0.55, 0.55, 0.6, 0.6, 0.65, 0.65, 0.7, 0.7, 0.75, 0.75, 0.80, 0.80, 0.85, 0.85, 0.9, 0.9, 0.9, 0.9, 0.9{]}                                                &                                               \\
\verb|inf_severe_sympt_prob| & {[}0.0001, 0.0001, 0.0001, 0.0001, 0.011, 0.011,  0.034, 0.034, 0.043, 0.043, 0.082, 0.082,  0.118, 0.118, 0.166, 0.166, 0.184, 0.184,  0.184, 0.184, 0.184{]}         &                                               \\
\verb|inf_severe_death_prob| & {[}0.00002, 0.00002, 0.00006, 0.00006, 0.0003, 0.0003, 0.0008,  0.0008, 0.0015, 0.0015, 0.006, 0.006, 0.022, 0.022, 0.051, 0.051, 0.093, 0.093, 0.093, 0.093, 0.093{]} &                                               \\
\verb|inf0_perc_symp|         & {[}0.5, 0.467, 0.033{]}                                                                                                                                                & Symptoms probabilities and population pyramid
\end{tabular}
\end{table}

==> supp_materials/COMORBUSS/chapters/ch04_interventions.tex <==
% Chapter 4
\chapter{Interventions} % Main chapter title
\label{Ch04} % For referencing the chapter elsewhere, use \ref{Ch00} 

\section{Non Pharmacological Interventions}
COMORBUSS encompasses various Non Pharmaceutical Intervention (NPI) models, such as
\begin{itemize}
    \item individualized quarantine;
    \item generalized lockdown;
    \item social isolation (reduction in social activity);
    \item service based interventions;
    \item contact tracing;
    \item testing campaigns.
\end{itemize}
The scenarios simulated in this study are based on the first wave of infection in Maragogi, hence services related to tourism are closed. The other standard NPI adopted in the base scenario is social isolation based on telephonic {\color{red}triangulation data processed by }to provide the daily percentage of people which stayed home. This is modelled by randomly selecting at the beginning of each simulation day the desired number of agents and confining them to their homes for that day. 

Standard testing policy is the sorological testing of symptomatic agents. Diagnosed agents are quarantined at home if presenting mild symptoms or are hospitalized if their symptoms are severe. Quarantines and hospitalizations are lifted when agents leave the infectious compartment by recovering or dying.

\subsection{Intervention in School Dynamics}
We implemented and combined the following NPIs in the context of schools:
\begin{itemize}
    \item reduced workload: daily teaching hours are reduced from 4 to 2 hours;
    \item alternating groups: students are separated into two groups which attend the classroom in alternating days;
    \item masks: students and professors are supplied masks with given penetration factors;
    \item active monitoring: suspicious cases are monitored and intermittent closing is declared upon discovery of cases
    \begin{itemize}
        \item suspicious cases are students, professionals or their relatives which present symptoms;
        \item suspicious cases are tested and if the diagnose is positive the student is quarantined;
        \item the classroom associated to the quarantined person is closed for 14 days;
        \item if using alternating groups, only the group associated to the quarantined person is suspended;
        \item if more than one classroom is closed in the span of a week, the whole school is closed for a week.
    \end{itemize}
\end{itemize}

The effects of these NPIs and their combinations are the main results of this work.

\subsection{Aerosol transmission model: masks and air exchange}
Interventions in the aerosol model are made via parametrization of the Equation \eqref{eq:edo_C}. We introduce values for the penetration factor of masks $p_m^i$ used by students and professionals, and test the efficacy of different scenarios under various values of volume flow rate $\Lambda$ of air with the exterior. For reference, we highlight documented or recommended values of these parameters.

\section{Vaccination Model}
The vaccination model used in this study is a simple binary model for infection. Vaccinated agents can become immune (susceptibility 0) with a probability given by the vaccine effectiveness after a given period. If the vaccination of an agent does not lead to immunity, its susceptibility remains unchanged. In the present work we assumed a worst case scenario where vaccines were not widely available and were prioritized to the teachers and staff. We assume that these professionals are already immune upon the reopening of the schools.

==> supp_materials/COMORBUSS/chapters/ch05_technical.tex <==
% Chapter 5
\chapter{Data and Code availability} % Main chapter title
\label{Ch05}

\section{Distribution and Documentation}
COMORBUSS has a project webpage under the link \href{https://comorbuss.org/}{https://comorbuss.org}, where all developments, results and links are assembled.

The source code for COMORBUSS is available in the repository \href{https://gitlab.com/ggoedert/comorbuss}{https://gitlab.com/ggoedert/comorbuss} under the licende \href{https://www.gnu.org/licenses/agpl-3.0.en.html}{AGPLv3}. The version of the code together with all required input files and simulation scripts is available under the Tag Paper\_Maragogi\_Schools.

The full documentation of the COMORBUSS library is available via \href{https://docs.comorbuss.org/}{https://docs.comorbuss.org/} under the license \href{https://creativecommons.org/licenses/by-sa/4.0/}{CC BY-SA 4.0}.

\section{Computing language and Dependencies}
Here we specify all the versions of the computer libraries used for the present work. COMORBUSS is written in Python (version 3.7.7) and requires the following modules:
\begin{itemize}
    \item numpy v.1.18
    \item matplotlib v.3.1.3
    \item pandas v.1.0.5
    \item seaborn v.0.10.1
    \item h5py v.3.10
    \item h5dict v.0.2.2
    \item scipy v.1.5.0
    \item portion v.2.0.2
    \item networkx v.2.5.1
    \item tqdm v.4.46.0
    \item numba v.0.53.1
\end{itemize}


%\section{Performance}

==> supp_materials/canada_schools/canada_schools.tex <==
\chapter{Canada schools}
\label{sec:canada_schools}

{\color{red} TO BE REMOVED: their model differs from ours, and a straight comparison cannot be made. For the purpose of justifying the $p_m$ values we used, it suffices to reference one of their tables}

==> supp_materials/closed_schools_baseline/closed_schools_baseline.tex <==
\chapter{Closed schools as baseline}
\label{sec:closed_schools_baseline}


==> supp_materials/networks_social_dynamics/networks_social_dynamics.tex <==
\chapter{Network social dynamics}
\label{sec:network_social_dynamics}

